US Microelectronics Packaging Ecosystem: Challenges and Opportunities

The semiconductor industry is experiencing a significant shift from traditional methods of shrinking devices and reducing costs. Chip designers actively seek new technological solutions to enhance cost-effectiveness while incorporating more features into the silicon footprint. One promising approach is Heterogeneous Integration (HI), which involves advanced packaging techniques to integrate independently designed and manufactured components using the most suitable process technology. However, adopting HI introduces design and security challenges. To enable HI, research and development of advanced packaging is crucial. The existing research raises the possible security threats in the advanced packaging supply chain, as most of the Outsourced Semiconductor Assembly and Test (OSAT) facilities/vendors are offshore. To deal with the increasing demand for semiconductors and to ensure a secure semiconductor supply chain, there are sizable efforts from the United States (US) government to bring semiconductor fabrication facilities onshore. However, the US-based advanced packaging capabilities must also be ramped up to fully realize the vision of establishing a secure, efficient, resilient semiconductor supply chain. Our effort was motivated to identify the possible bottlenecks and weak links in the advanced packaging supply chain based in the US.

==> figures/makefigs.tex <==
\let\oldincludegraphics\includegraphics
\newcommand{\dummyincludegraphics}[2][]{}

\newcommand{\hidegraphics}{\let\includegraphics\dummyincludegraphics}
\newcommand{\unhidegraphics}{\let\includegraphics\oldincludegraphics}

\newcommand{\testfig}{
\begin{figure}
\centering
\includegraphics[width=0.6\textwidth]{figures/fig1.png}
\caption{}
\label{fig:testfig}
\end{figure}
}

==> packaging_needs_table.tex <==

\begin{table*}[ht!]
\caption{US-based advanced packaging supply chain needs and capabilities}
\label{Table comparison}
\centering
\begin{tabular}{|c|c|c|c|c|c|}
%\includegraphics[height = 4cm, width = 4cm]{Screenshot 2022-12-11 at 3.16.52 AM.png}

    \hline
            \textbf{\thead{Application field}} & \textbf{\thead{Requirements}}  & \textbf{\thead{Type of packaging\\ technology}} & \textbf{\thead{Offshore\\ dependency}}& \textbf{\thead{US-based \\IDM/OSATs}} & \textbf{\thead{Dependencies\\ and issues}}\\
    \hline
            \thead{Aerospace and Defense} & \thead{Durability, \\reliability,\\security} & \thead{AiP, RADAR packaging}  & Low  &\thead{Qoorvo,\\Honeywell,\\Northrop Gruman} &\thead{Secured by 83 trusted\\ onshore suppliers,\\high manufacuring\\cost,\\low volume} \\
    \hline
            \thead{5G Communication} & \thead{High frequency\\ operation, beamforming} &  \thead{legacy packaging, \\AiP} & Medium & \thead{Qoorvo,\\ Analog Devices,\\Skyworks} & \thead{Substrate \\dependency}  \\
    \hline
            \thead{High-Performance\\ Computing} & \thead{High data rates and\\memory bandwidth} & 2.5D, 3D & High & \thead{Intel}&\thead{Highly dependent on\\ offshore IDM and OSATs\\ like TSMC\\ for advance node} \\
    \hline
             \thead{Automotive} & \thead{Integration of sensors,\\ MEMS, LiDAR\\ \& RADAR packaging} & \thead{legacy packaging,\\ 2.5D, 3D packaging} & High & \thead{Velodyne,\\Innovusion} &\thead{Substrate dependency, \\ significant offshore \\ dependency for LiDAR\\packaging }  \\
    \hline
             \thead{Internet of Things (IoT)} & \thead{Low power, \\small form factor,\\sensor integration} & FOWLP & High & \thead{Texas Instrument,\\Marvell}& \thead{High offshore\\dependency}\\
    \hline
             \thead{Mobile} & \thead{Low power, \\small form factor} & PoP, WLP, Stacked die &  High&\thead{Skyworks,\\ Qoorvo} & \thead{Highly dependent on\\ offshore IDM and OSATs\\ like TSMC\\ for advance node} \\
    \hline
            \thead{Medical and Health} &\thead{Flexible, \\biodegradable \\packaging}  & WLP, FCBGA & High & \thead{Analog Devices} & Substrate dependency \\
    \hline
     %       \thead{Silicon Photonics} &  & &   &\\
   % \hline
\end{tabular}
\end{table*}

==> sections/background.tex <==
\section{background}


\subsection{Motivation of Heterogenous Integration (HI)}



\subsection{Challenges of HI}



\subsection{Advanced Packaging for HI}



\subsection{Current System in Package (SiP) Supply Chain}




==> sections/introduction.tex <==
\section{Introduction}
The integration of electronic devices into our daily lives is having a profound impact, completely transforming our lifestyles and work processes. We now exist within a digital economy where high-speed and interconnected devices generate massive amounts of data. This data is crucial for enabling transactions in various sectors such as autonomous vehicles, data centers, and artificial intelligence systems. However, effectively processing this big data requires systems that can capture, store, and analyze it. This is where state-of-the-art semiconductor integrated circuits (ICs) come into play. These advanced ICs possess multiple processing cores, high-speed memory, and efficient input/output capabilities. They have been made possible by Moore's law, which has driven the semiconductor industry to produce ICs that are faster, smaller, and more affordable over time. However, the continued application of Moore's law is facing challenges due to rising fabrication costs, power consumption issues, and lower yields at advanced technology nodes. To address these challenges, the International Technology Roadmap for Semiconductors (ITRS) introduced a long-term vision in 2015 called Heterogeneous Integration (HI). HI involves the integration of individually designed and fabricated components on an interposer substrate, resulting in a System in Package (SiP). Please refer to Figure 1 for an illustration of how heterogeneous integration builds a SiP. Through heterogeneous integration, different components from various technology nodes and functionalities are brought together to form a higher-level assembly known as a SiP or Multi-Chip Module (MCM). SiPs offer enhanced functionality and improved operational characteristics that are difficult to achieve with a single die system-on-chip (SoC). Within a SiP, various components like chiplets, MEMS devices, and active/passive parts are integrated into a single package. Chiplets are individual silicon dies specifically designed for functions such as memory, analog-mixed signal processing, RF communication, or processing tasks. The system-in-package can be realized through vertical stacking (3D) or adjacent placement (2.5D) of chiplets on the interposer substrate. Many key players in the industry, including integrated device manufacturers like Intel, Micron, and Samsung, fabless design houses like AMD and IBM, foundries like TSMC, and outsourced semiconductor assembly and testing companies like TSMC and Amkor, are actively involved in developing solutions for heterogeneous integration. For example, commercially available examples of heterogeneous 3D system-in-packages (SiPs) include Intel Agilex and AMD EPYC. The Defense Advanced Research Projects Agency (DARPA) shares a similar vision for the United States Department of Defense (DoD) applications. To promote trusted microelectronics designs and technologies, DARPA is driving the Common Heterogeneous Integration and IP Reuse Strategies (CHIPS) program.
